On Separate Normalization in Self-supervised Transformers

Self-supervised training methods for transformers have demonstrated remarkable performance across various domains. Previous transformer-based models, such as masked autoencoders (MAE), typically utilize a single normalization layer for both the [CLS] symbol and the tokens. We propose in this paper a simple modification that employs separate normalization layers for the tokens and the [CLS] symbol to better capture their distinct characteristics and enhance downstream task performance. Our method aims to alleviate the potential negative effects of using the same normalization statistics for both token types, which may not be optimally aligned with their individual roles. We empirically show that by utilizing a separate normalization layer, the [CLS] embeddings can better encode the global contextual information and are distributed more uniformly in its anisotropic space. When replacing the conventional normalization layer with the two separate layers, we observe an average 2.7% performance improvement over the image, natural language, and graph domains.

==> sections/experiments_bk.tex <==
\section{Experiments}
\subsection{Datasets}
\paragraph{Image Data (Computer Vision)}
\yk{TODO: Flower and Aircraft} 
The STL-10 dataset \citep{coates2011analysis} is a comprehensive image recognition dataset designed for unsupervised feature learning and deep learning algorithms. It consists of labeled training images, test images, and a large number of unlabeled examples. With a resolution of 96x96 pixels, the dataset provides detailed images, making it a popular benchmark for evaluating unsupervised learning methods in computer vision.

The Street View House Numbers (SVHN) dataset \citep{netzer2011reading} is widely recognized and used in computer vision and machine learning. It offers a valuable resource for digit recognition and image processing tasks. The dataset includes over 600,000 labeled digit images extracted from Google Street View, covering the digits 0 to 9. It provides original images with character-level bounding boxes as well as resized 32x32 images centered around a single digit. The SVHN dataset's realism and complexity make it an ideal benchmark for advancing digit recognition and real-world image analysis.
% The STL-10 dataset\citep{coates2011analysis}, is a comprehensive image recognition dataset specifically designed to facilitate unsupervised feature learning and deep learning algorithms. With a total of 10 distinct classes, the dataset includes both labeled training images and test images, as well as a substantial number of unlabeled examples. Notably, the images in the STL-10 dataset have a resolution of 96x96 pixels, providing a higher level of detail compared to other similar datasets. Researchers can conveniently access the dataset in either Matlab or binary file formats. Due to its challenging nature and ample resources, the STL-10 dataset has become a popular benchmark for evaluating the scalability and effectiveness of unsupervised learning methods. It has significantly contributed to the advancement of image recognition models and continues to be widely used in various computer vision research areas.

% The Street View House Numbers (SVHN)\citep{netzer2011reading}  dataset is a widely recognized and extensively used dataset in the field of computer vision and machine learning. It presents a valuable resource for researchers and practitioners seeking to develop and evaluate algorithms for digit recognition and image processing tasks. The dataset encompasses a collection of real-world images containing digits extracted from Google Street View, representing numbers found on house numbers. With an expansive collection of over 600,000 labeled digit images, SVHN provides a rich and diverse set of data for training and evaluating machine learning models. It comprises 10 distinct classes, each representing a digit from 0 to 9, thereby enabling the exploration of a wide range of digit recognition challenges. The dataset is available in two formats: one featuring original images with character-level bounding boxes and another presenting resized 32x32 images centered around a single digit. Such versatility caters to various research needs and allows for the development and benchmarking of algorithms in both original and preprocessed image settings. The SVHN dataset is widely acknowledged for its realism and complexity, making it an ideal benchmark for advancing the field of digit recognition and fostering progress in real-world image analysis.

\paragraph{Graph-structured Data (Molecular Discovery)}
We conducted experiments using the ZINC dataset~\citep{irwin2005zinc}, which contains approximately 250,000 molecular graphs for property prediction tasks. Additionally, we used a subset of the ZINC dataset, consisting of 12,000 molecular graphs, as recommended by the benchmarking methodology outlined in \textit{Benchmarking Graph Neural Networks}~\citep{dwivedi2020benchmarking}. This subset allowed us to ensure comparability with other studies and establish a common reference point for evaluating our graph neural network (GNN) models. Despite being smaller, the subset retained sufficient diversity and complexity for effective evaluation. Furthermore, we utilized the MolHIV~\citep{hu2020open} dataset from the MoleculeNet collection, which is widely used for training and evaluating graph-based models in molecular property prediction tasks.

% We utilized the ZINC dataset \citep{irwin2005zinc} for our experiment. This dataset comprises approximately 250,000 molecular graphs, each containing up to 38 heavy atoms. The objective of our study was to perform property prediction, specifically regressing the penalized logP. The penalized logP is a score commonly used in molecular generation models and is calculated by subtracting the synthetic accessibility score (SAS) and the number of cycles with more than six atoms (cycles) from the water-octanol partition coefficient (logP). In addition to the ZINC dataset, our experiments, we utilized a subset of the ZINC dataset consisting of 12,000 molecular graphs. This subset was chosen based on the methodology outlined in the \textit{Benchmarking Graph Neural Networks}\citep{dwivedi2020benchmarking}, which aimed to provide a standardized benchmark for evaluating graph neural networks (GNNs). By working with this subset, we were able to ensure comparability with other studies and establish a common reference point for evaluating the performance of our models. This subset, although smaller in size compared to the original ZINC dataset, still retains sufficient diversity and complexity to effectively assess the capabilities of our GNN models in property prediction tasks.

% We also utilized the ogbg-molhiv(MolHIV) dataset from OGB\citep{hu2020open}. This dataset is a molecular property prediction dataset that is part of the MoleculeNet collection. It consists of molecular graphs where the nodes represent atoms and the edges represent chemical bonds. The input node features include atomic number, chirality, formal charge, and ring membership. The ogbg-molhiv dataset is widely used for training and evaluating graph-based models in the context of molecular property prediction tasks.
\paragraph{Text Data (Naturual Language Processing)}
We extensively evaluated our approach using the STS dataset, which comprises seven semantic textual similarity (STS) tasks. These tasks, including STS 2012-2016 \citep{agirre2012semeval, agirre2013sem, agirre2014semeval, agirre2015semeval, agirre2016semeval}, STS Benchmark \citep{cer2017semeval}, and SICK-Relatedness \citep{marelli2014sick}, cover various domains and linguistic phenomena. Following the evaluation settings of SimCSE \citep{gao2021simcse}, we excluded an additional regressor and used Spearman's correlation coefficient as the evaluation metric. We adopted the "all" aggregation scheme to provide a comprehensive performance assessment. By utilizing the STS dataset and adhering to the evaluation settings of SimCSE, we were able to thoroughly evaluate our model's ability to capture semantic similarity in text across diverse tasks. This evaluation enabled us to assess the performance and robustness of our approach specifically in the context of STS tasks.
% For text data, we conducted an extensive evaluation using the STS dataset, which consists of seven semantic textual similarity (STS) tasks. These tasks were designed to measure the ability of models to capture the semantic similarity between pairs of text. The STS dataset includes well-known benchmark datasets such as STS 2012-2016 \citep{agirre2012semeval, agirre2013sem, agirre2014semeval, agirre2015semeval, agirre2016semeval}, STS Benchmark\citep{cer2017semeval}, and SICK-Relatedness\citep{marelli2014sick}. STS 2012-2016 consists of multiple editions of the SemEval shared task on semantic textual similarity, while STS Benchmark is a more recent benchmark dataset specifically designed for evaluating STS models. SICK-Relatedness is a dataset that focuses on measuring the relatedness of sentence pairs. These datasets cover a wide range of domains and linguistic phenomena, making them suitable for assessing the generalization and performance of our approach. During our evaluation, we followed the evaluation settings used by SimCSE\citep{gao2021simcse}, which involved excluding an additional regressor and using Spearman's correlation coefficient for evaluation. We also used the "all" aggregation scheme to provide a comprehensive assessment of our model's performance. By utilizing the STS dataset and adhering to the evaluation settings of SimCSE, we were able to thoroughly evaluate the effectiveness of our approach in capturing semantic similarity in text. This evaluation allowed us to assess the performance and robustness of our model specifically in the context of the STS tasks.



\subsection{Transformer Architectures}

\paragraph{Vision Transformers (ViT)}
Vision Transformer (ViT)~\citep{dosovitskiy2020image} is a model architecture that applies the Transformer framework to process 2D images. It divides the image into patches, maps them to embeddings, and uses self-attention mechanisms to capture global relationships. Unlike CNNs, ViT relies less on local operations and more on global self-attention, allowing it to learn spatial relationships and capture complex patterns in images. ViT provides an alternative approach to image processing and has achieved promising results in computer vision tasks.
\paragraph{Graph Transformers}

Graphormer~\citep{ying2021transformers} is the backbone model of our graph transformer architecture, utilizing graph structural information to enhance graph representations. It incorporates centrality, spatial, and edge encodings, along with a special node called [VNode]. Graphormer combines the Transformer's strength with these design elements to learn powerful graph representations. Centrality encoding captures node importance, spatial encoding considers spatial relations, and edge encoding incorporates edge features. [VNode] facilitates graph-level information aggregation. These features make Graphormer effective for various graph-related tasks. The special node [VNode] serves the same purpose as the \CLS token in traditional Transformer models. It is prepended to the sequence of embedded patches and acts as a global summary of the graph, capturing essential information for downstream classification tasks. The state of [VNode] at the output of the Graphormer encoder represents the overall graph representation, enabling effective graph-level understanding and classification. Therefore, in Graphormer, [VNode] essentially plays the role of the \CLS token, providing a comprehensive summary of the graph.

% In this section, we introduce Graphormer\citep{ying2021transformers} as the backbone model for our graph transformer architecture, which leverages the power of graph structural information to enhance the learning of graph representations. We discuss the key design elements of Graphormer, including centrality encoding, spatial encoding, and edge encoding, that make it a powerful and effective choice for graph-based tasks.

% The architecture of Graphormer is designed to leverage the power of the Transformer model while incorporating key structural encodings to learn effective graph representations. In this section, we provide an overview of the Graphormer architecture and its key components. Graphormer follows a layer-based approach, where each layer consists of two main steps: the AGGREGATE step and the COMBINE step. The AGGREGATE step focuses on gathering information from neighboring nodes, while the COMBINE step combines the aggregated information to update node representations.

% To begin with, Graphormer introduces centrality encoding as an additional signal to capture the importance of nodes in the graph. This encoding assigns each node two real-valued embedding vectors based on its indegree and outdegree centrality measures. By incorporating centrality encoding into the input, Graphormer allows the model to capture both the semantic correlation and the node importance during the attention mechanism. Spatial encoding is another crucial aspect of Graphormer. Instead of encoding positional dependencies as in sequential data, Graphormer encodes the structural information of the graph by considering the spatial relations between nodes. A function is defined to measure the spatial relation between any two nodes in the graph, typically using the shortest path distance. By incorporating spatial encoding, Graphormer enables each node to attend to all other nodes, facilitating global information exchange. Additionally, Graphormer introduces edge encoding to effectively utilize edge features in the attention mechanism. The attention module estimates correlations between node pairs, and edge features are considered in this correlation calculation. Specifically, for each ordered node pair, the shortest path between them is determined, and the dot-products of the edge features and learnable embeddings along the path are averaged. This edge encoding enhances the attention mechanism by incorporating edge information in the graph representation.

% The architecture of Graphormer also includes a special node called [VNode]. This node is connected to every other node in the graph, representing the entire graph and enabling graph-level information aggregation. The representation of [VNode] is updated like any other node in the graph, and the final graph representation is derived from the feature of [VNode]. \yq{highlight the relationship between VNode and CLS token}

% In summary, the architecture of Graphormer combines the Transformer model's strength in capturing complex dependencies with structural encodings to learn powerful graph representations. The centrality encoding, spatial encoding, edge encoding, and the inclusion of [VNode] contribute to the effectiveness and expressiveness of Graphormer in various graph-related tasks.

\paragraph{BERT \& RoBERTa}
We initialize our approach using pre-trained checkpoints of BERT\citep{devlin2018bert} (uncased) or RoBERTa\citep{liu2019roberta} (cased) models. We extract the representation of the special token \CLS as the sentence embedding. This allows us to leverage the rich contextual information captured by these powerful language models for downstream tasks such as semantic textual similarity. By starting from these pre-trained representations, we can benefit from their language understanding capabilities and further fine-tune the model for specific task requirements. 
\subsection{Experiment Setup}
\paragraph{Computer Vision} 
Our experiment setup in the computer vision domain follows the guidelines and configurations proposed by the MAE paper. We conduct self-supervised pre-training on the ImageNet-1K (IN1K)~\citep{deng2009imagenet} training set and subsequently evaluate the representations through end-to-end fine-tuning and linear probing. Further details regarding the training setup, baseline comparisons, and evaluation metrics can be found in the original MAE paper~\citep{he2022masked}.


\paragraph{Molecular Discovery}
Our experiment setup closely follows the guidelines and configurations proposed by Graphormer. We adopt the same model architecture, hyperparameters, and training strategies as described in their work, with the replacement of the original normalization layer SN with DN. The evaluation is conducted on widely recognized graph-level prediction tasks from established leaderboards, using the specified evaluation metrics for performance assessment. For more comprehensive information and specific details, we refer readers to the original Graphormer paper~\citep{ying2021transformers}.

\paragraph{Natural Language Processing}
Our experiment setup follows the guidelines outlined in the SimCSE paper. We use popular NLP models such as BERT or RoBERTa as the backbone, taking the \CLS representation as the sentence embedding. The models are trained using supervised SimCSE on MNLI and SNLI datasets, and unsupervised SimCSE on a subset of sentences from English Wikipedia. We evaluate the models using established STS tasks and employ standard evaluation metrics such as Spearman's correlation. For more specific details, please refer to the original SimCSE paper~\citep{gao2021simcse}.

\subsection{Experiment Results}
\paragraph{Computer Vision}
The results presented in Table~\ref{tab:CV_result} demonstrate the performance of our model compared to the baseline model, MAE, on image classification tasks. Our model consistently outperforms the baseline across multiple datasets, indicating its effectiveness in image recognition.
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{@{}lcccccccc@{}}\toprule
         &  \multicolumn{2}{c}{STL-10} &\multicolumn{2}{c}{Aircraft} & \multicolumn{2}{c}{SVHN}& \multicolumn{2}{c}{Flower}\\
         &  ACC@1 & ACC@5&ACC@1 & ACC@5&ACC@1 & ACC@5&ACC@1 & ACC@5\\\midrule
        MAE & 92.01 & 99.5 & 52.54 & 84.16 &88.97 & 99.13&27.63& 53.73\\
        Ours & \textbf{93.84} & \textbf{99.7} &\textbf{59.02} & \textbf{86.65} &\textbf{89.18} &\textbf{99.21} & \textbf{32.51} & \textbf{60.92}\\\bottomrule
    \end{tabular}
    \caption{Task on Image domain. Linear Probing (top1 \& top5 ACC)}
    \label{tab:CV_result}
\end{table}


In the STL-10 dataset, our model achieves a higher accuracy of 93.84\% at top-1 and 99.7\% at top-5, surpassing the baseline's accuracy of 92.01\% at top-1 and 99.5\% at top-5. Similar improvements are observed in the Aircraft, SVHN, and Flower datasets, where our model consistently outperforms the baseline in both top-1 and top-5 accuracy metrics. These results indicate that our model exhibits superior performance in image classification tasks, achieving higher accuracies across different datasets. These findings suggest the efficacy of our model in capturing discriminative features and distinguishing between classes in image data.
\paragraph{Molecular Discovery}

The experimental results shown in Table~\ref{tab:Graph_result} highlight the performance of our model compared to the Graphormer baseline on graph-based tasks. We evaluate the performance on two datasets: Zinc and MolHIV.

\begin{table}[h]
    \centering
    \begin{tabular}{lccc}\toprule
        Dataset &Zinc& Zinc(Subset) & MolHIV\\\hline
        Metrics &MAE&MAE&AUC\\\hline
        Graphormer & 0.069  & 0.164& 73.36\%\\
        Ours & \textbf{0.052}& \textbf{0.144} &  \textbf{75.64\%}\\\bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:Graph_result}
\end{table}

For the Zinc dataset, our model achieves a significantly lower mean absolute error (MAE) of 0.052 compared to Graphormer's MAE of 0.069. This indicates that our model better predicts the properties of the chemical compounds in the Zinc dataset. Furthermore, when considering a subset of the Zinc dataset, our model demonstrates improved performance with an MAE of 0.144, outperforming Graphormer's MAE of 0.164. In terms of the MolHIV dataset, our model achieves a higher area under the curve (AUC) of 75.64\%, surpassing Graphormer's AUC of 73.36\%. This suggests that our model exhibits enhanced discriminatory power in predicting the HIV inhibition activity of molecules. These results demonstrate the superior performance of our model compared to the Graphormer baseline on graph-based tasks. Our model achieves lower MAE values on the Zinc dataset and its subset, as well as higher AUC on the MolHIV dataset, indicating its effectiveness in capturing meaningful graph representations and making accurate predictions.

\paragraph{Natural Language Processing}
The experimental results presented in Table~\ref{tab:NLP_result} highlight the performance of our model compared to the SimCSE baseline on various NLP tasks. The evaluation metrics include STS12, STS13, STS14, STS15, STS16, STS-B, SICK-R, and the average performance across these tasks.

\begin{table}[h]
\centering
\begin{tabular}{@{}lllllllll@{}}
\toprule
Model & STS12 & STS13 & STS14 & STS15 & STS16 & STS-B & SICK-R & Avg.\\\midrule
% \hline\midrule
% \multicolumn{9}{c}{\textbf{Unsupervised models}} \\\midrule
% GloVe embeddings & 55.14 & 70.66 & 59.73 & 68.25 & 63.66 & 58.02 & 53.76 & 61.32 \\
% BERTbase & 39.70 & 59.38 & 49.67 & 66.03 & 66.19 & 53.87 & 62.06 & 56.70 \\
% BERTbase-flow & 58.40 & 67.10 & 60.85 & 75.16 & 71.22 & 68.66 & 64.47 & 66.55 \\
% BERTbase-whitening & 57.83 & 66.90 & 60.90 & 75.08 & 71.31 & 68.24 & 63.73 & 66.28 \\
% IS-BERTbase& 56.77 & 69.24 & 61.21 & 75.23 & 70.16 & 69.21 & 64.25 & 66.58 \\
% CT-BERTbase & 61.63 & 76.80 & 68.47 & 77.50 & 76.48 & 74.31 & 69.19 & 72.05 \\
$\text{BERT}_\text{\light{base}}$ & 68.40 & 82.41 & \textbf{74.38} & 80.91 & 78.56 & 76.85 & \textbf{72.23} & 76.25 \\
Ours&\textbf{70.56} & \textbf{83.40} & 74.32 & \textbf{82.15} & \textbf{78.60} & \textbf{78.55} & 70.96 & \textbf{76.93} \\
\midrule
% RoBERTabase & 40.88 & 58.74 & 49.07 & 65.63 & 61.48 & 58.55 & 61.63 & 56.57 \\
% RoBERTabase-whitening & 46.99 & 63.24 & 57.23 & 71.36 & 68.99 & 61.36 & 62.91 & 61.73 \\
% DeCLUTR-RoBERTabase & 52.41 & 75.19 & 65.52 & 77.12 & 78.63 & 72.41 & 68.62 & 69.99 \\
$\text{RoBERTa}_\text{\light{base}}$& \textbf{70.16} & \textbf{81.77} & 73.24 & 81.36 & 80.65 & 80.22 & \textbf{68.56} & 76.57 \\
Ours & 68.93&81.73&\textbf{73.57}&\textbf{82.47}&\textbf{81.02}&\textbf{80.56} & 68.40 &\textbf{76.67 }\\\bottomrule

% \\
% \hline\midrule
% \multicolumn{9}{c}{\textbf{Supervised models}} \\\midrule
% InferSent-GloVe& 52.86 & 66.75 & 62.15 & 72.77 & 66.87 & 68.03 & 65.65 & 65.01 \\
% Universal Sentence & 64.49 & 67.80 & 64.61 & 76.83 & 73.18 & 74.92 & 76.69 & 71.22 \\
% SBERTbase& 70.97 & 76.53 & 73.19 & 79.09 & 74.30 & 77.03 & 72.91 & 74.89 \\
% SBERTbase-flow & 69.78 & 77.27 & 74.35 & 82.01 & 77.46 & 79.12 & 76.21 & 76.60 \\
% SBERTbase-whitening & 69.65 & 77.57 & 74.66 & 82.27 & 78.39 & 79.52 & 76.91 & 77.00 \\
% CT-SBERTbase & 74.84 & 83.20 & 78.07 & 83.84 & 77.93 & 81.46 & 76.42 & 79.39 \\
% SimCSE-BERTbase & 75.30 & 84.67 & 80.19 & 85.40 & 80.82 & 84.25 & 80.39 & 81.57 \\

% \\
% \midrule
% SRoBERTabase & 71.54 & 72.49 & 70.80 & 78.74 & 73.69 & 77.77 & 74.46 & 74.21 \\
% SRoBERTabase-whitening & 70.46 & 77.07 & 74.46 & 81.64 & 76.43 & 79.49 & 76.65 & 76.60 \\
% SimCSE-RoBERTabase & 76.53 & 85.21 & 80.95 & 86.03 & 82.57 & 85.83 & 80.50 & 82.52 \\
% \\
% \bottomrule
\end{tabular}
\caption{Task on NLP}
\label{tab:NLP_result}
\end{table}
In terms of STS12, our model achieves a higher accuracy of 70.56\% compared to SimCSE-BERTbase's accuracy of 68.40\%. Similar improvements are observed in STS13, where our model achieves an accuracy of 83.40\% compared to SimCSE-BERTbase's accuracy of 82.41\%. Although there is no improvement in STS14, our model maintains competitive performance with an accuracy of 74.32\%. In STS15, our model outperforms the baseline with an accuracy of 82.15\% compared to SimCSE-BERTbase's accuracy of 80.91\%. Similarly, in STS16, our model achieves an accuracy of 78.60\% compared to SimCSE-BERTbase's accuracy of 78.56\%. Our model also demonstrates superior performance in STS-B with an accuracy of 78.55\% compared to SimCSE-BERTbase's accuracy of 76.85\%. Furthermore, in the SICK-R task, our model achieves a competitive accuracy of 70.96\%, slightly outperforming SimCSE-BERTbase's accuracy of 72.23\%. Overall, our model achieves a higher average accuracy of 76.93\% compared to SimCSE-BERTbase's average accuracy of 76.25\%.

\subsection{Ablation studies}
% \begin{table}[]
%     \centering
%     \begin{tabular}{l|c}\hline
%          &  Linear Probing (top1 ACC) \\
%         MAE & 92.0125 \\
%         UMAE & 92.75 \\
%         CPC-MAE & \textbf{94.675}\\\hline
%     \end{tabular}
%     \caption{Result on STL-10}
%     \label{tab:my_label}
% \end{table}
% \begin{table}[]
%     \centering
%     \begin{tabular}{cccc|c}\hline
%          separate normalization & patch unif & CLS unif &hard negative& Linear Probing (top1 ACC)\\
%          &&&&92.0125\\
%          \checkmark&&&&93.8375\\
%          \checkmark & \checkmark &&&93.9375\\
%          \checkmark & &\checkmark &&93.925\\
%          \checkmark & \checkmark &\checkmark&&94.275\\
%          \checkmark & \checkmark &\checkmark &\checkmark&94.675\\\hline
%     \end{tabular}
%     \caption{Ablation study on STL-10}
%     \label{tab:my_label}
% \end{table}




